OS-Marathon: Benchmarking Computer-Use Agents on Vast-Horizon, Repetitive Tasks

Vast-horizon, repetitive workflows are common in daily routines, e.g., processing expense reports from a stack of receipts, organising a collection of PDF annotations into structured notes, and are tedious for humans, with execution length scaling with the volume of data to process. They are, however, well-suited to autonomous agents, since their structured, recurring sub-workflows follow a logic that can be systematically learned. Yet no existing benchmark evaluates agents specifically on vast-horizon, repetitive capabilities, leaving the problem largely underexplored. To bridge this gap, we establish OS-Marathon, comprising 100 vast-horizon, repetitive tasks across 5 scenarios and 10 domains, on which our evaluation reveals that leading state-of-the-art (SOTA) CUAs struggle substantially. We further find that introducing a task orchestrator to decompose the workflow into per-instance subtasks fails to mitigate the challenge: errors accumulate and propagate across solver agents, indicating that naive decomposition is insufficient for these tasks. We then explore a cost-friendly personalisation strategy, i.e. GraphDemo, that adapts general agents to such tasks from a single human demonstration of the recurring sub-workflow logic. Extensive experiments show both the real-world challenge of vast-horizon, repetitive tasks and the improvement provided by human demonstration in this setting. Project website: https://os-marathon.github.io/.

==> commands.tex <==
\usepackage{xspace}
\newcommand{\ourbenchmark}{OS-Marathon\xspace}
\newcommand{\ourbenchmarklite}{OS-Marathon-Lite\xspace}
\newcommand{\ourbenchmarkpro}{OS-Marathon-Pro\xspace}
\newcommand{\tasknum}{100\xspace}
\newcommand{\subtasknum}{849\xspace}
\newcommand{\scenarionum}{5\xspace}
\newcommand{\domainnum}{10\xspace}
\newcommand{\envnum}{12\xspace}
\newcommand{\atomictypenum}{18\xspace}
\newcommand{\atomictaskcategories}{6\xspace}
\newcommand{\etc}{etc.\@\xspace}
\newcommand{\inlinelogo}[1]{\raisebox{-0.2ex}{\includegraphics[height=1em]{#1}}}

% Color-coding macros
\usepackage{xcolor}
\usepackage{soul}
\usepackage{etoolbox}
\newtoggle{draft}\toggletrue{draft}
\newcommand{\new}[1]{\iftoggle{draft}{\textcolor{blue}{#1}}{#1}}
\newcommand{\revised}[1]{\iftoggle{draft}{\textcolor{orange}{#1}}{#1}}
\newcommand{\todo}[1]{\iftoggle{draft}{\textcolor{red}{\textbf{[TODO: #1]}}}{}}
\newcommand{\note}[2]{\iftoggle{draft}{\textcolor{purple}{[#1: #2]}}{}}
\newcommand{\hlt}[1]{\iftoggle{draft}{\hl{#1}}{#1}}
\newcommand{\wenjie}[1]{\iftoggle{draft}{\textcolor{teal}{[Wenjie: #1]}}{}}
